Reasoning About Knowledge on Regular Expressions is 2EXPTIME-complete

Logics for reasoning about knowledge and actions have seen many applications in various domains of multi-agent systems, including epistemic planning. Change of knowledge based on observations about the surroundings forms a key aspect in such planning scenarios. Public Observation Logic (POL) is a variant of public announcement logic for reasoning about knowledge that gets updated based on public observations. Each state in an epistemic (Kripke) model is equipped with a set of expected observations. These states evolve as the expectations get matched with the actual observations. In this work, we prove that the satisfiability problem of $\POL$ is 2EXPTIME-complete.

==> sectionrelatedworks_copy.tex <==
\newcommand{\CTLK}{\textsf{CTLK}}
\textbf{Propositional Dynamic Logics.} In $\POL$, a residuated model $\M|_w$ can have at most a unique successor $\M|_{wa}$ for a letter $a$ in the alphabet. This gives rise to a $\Sigma$-labelled transition structure equivalent to a model where each node is an epistemic skeleton of some $\M|_w$. 
% In this work, we have shown that the Public Observation Logic is decidable. In doing so, we have came across connections and similarities regarding the structures and the expressivity of other logical systems. Each state in a $\POL$ model is equipped with a regular expression. If we look at the proof of Theorem \ref{algo-correct}, we prove equivalence between a $\POL$ model and a finite transition structure, whose nodes intuitively correspond to the epistemic skeleton of some $\POL$ models, $\M|_w$, where $w\in\Sigma^*$.It can be seen that such a structure would have, for each node, at most one transition labelled for each letter in $\Sigma$. 
Thus we get a natural connection with a Deterministic Propositional Dynamic Logic (DPDL) \cite{dpdlbenari82} model structure. But, there is a significant difference: each node in our constructed transition structure is an epistemic model, whereas in DPDL, it is a propositional valuation. To the best of our knowledge, no such deterministic structures involving epistemic constructions have been studied beforehand. 

Epistemic Propositional Dynamic Logic (EPDL) has been studied in \cite{epdlli18}. As in $\POL$, each node of an EPDL model is an epistemic structure, and it assumes \emph{perfect recall}. However, the transitions in EPDL are non-deterministic ones. Moreover, in EPDL, valuations may change when actions are executed, while that is not the case when observations are made in POL.

%The most important difference here constitutes the notion of valuation and overall epistemic structure. To be precise, in our case, when a model is residuated or projected, the surviving nodes remain the same except for the expectation expressions getting revised, thus keeping the propositional valuations intact. 
%However, in EPDL, the epsitemic model that is transitioned to, can be arbitrary, satisfying only some transition conditions. %keeping only Perfect Recall and No Miracles consistent with it. 

Another study on a PDL-like logic with epistemic operators \cite{heinemannpdlk07} concerns single agent knowledge formulas, where, verification of \textit{only} knowledge formulas in the regular expressions is considered. Although, they have given a hardness result (EXPTIME-hard) that follows from PDL, they do not have any matching upper bound. 

\noindent\textbf{Temporal Logics.} Since we are dealing with sequences of observations and how the expected observation expressions get residuated, there is a subtle temporal aspect to $\POL$. %We explored such a connection with $\LTLK$ \cite{ltlkhalpern} in the previous section. 
In $\LTLK$, the interaction between time and knowledge assumes \emph{perfect recall} and \emph{synchronous} rules, which also hold in $\POL$. % - a technical discussion is  %Yet, among being different on consistent valuations and the way epistemic model is updates, it is also 
But, there are some differences in the \textit{linearity} aspects. More precisely, since $\POL$ deals with multiple letters in the transition alphabet, knowledge does not change linearly, in the sense that, knowledge can change depending on the observations that occur. At a single point of occurrence this can be any one of the letters in the alphabet. We note here that a valuation in a state in the next temporal transition in $\LTLK$ may change, whereas such a valuation remains consistent in POL. Thus, $\neg p \land X p$ is satisfiable in $\LTLK$, whereas $\neg p \land \langle a\rangle p$ is not satisfiable in $\POL$, which leads to a difference in expressive power. From the complexity viewpoint, the satisfiability problem of $\LTLK$ is non-elementary, whereas for  $\POL$, it is $\mathsf{2EXPTIME}$-complete. It is interesting to note that both $\LTLK$ and $\POL$ can express that \emph{after some finite sequence of observations, $\varphi$ holds}, but only $\POL$ can express that \emph{after some even occurrences of observations, $\phi$ holds}. Resolving the intricate relationship between $\LTLK$ and $\POL$ needs further study.
%Another major difference between $\POL$ and such Epistemic LTL systems lies in expressive power. 
% (Since $\POL$ involves regular expressions, it can express more than these temporal systems of knowledge, even the $\POL$ with single letter. For example, even though both Epistemic LTL and $\POL$ with single letter can express the fact that "after some finite observation some fact $\phi$ holds", only $\POL$ with single letter can express the fact that "after some \textit{even} occurrences of observations some fact $\phi$ holds".)

Since knowledge updates \textit{branch out} in $\POL$ depending upon the action observed, Computational Tree Logic with epistemic operators ($\CTLK$) \cite{ctlkdima08} forms a close neighbour, whose satisfiability problem turns out to be undecidable. We note here that unravelled $\POL$ models create indistinguishability within the nodes (distinct $\POL$ models) themselves, whereas, indistinguishability in a $\CTLK$ model occurs among nodes across the tree. %a node in a \CTLK model is a possible state with indistinguishability across the tree. 

%\noindent\textbf{Public Announcement Logics.} $\POL$ is quite similar to Public Announcement Logic ($\PAL$) as well (see \cite{krpolsf23} for a detailed comparison). $\PAL$ with Kleene-star (operators of the form $[\phi^*]\psi$: after announcing $\phi$ publicly a finite number of times, $\psi$ holds) has been shown to be undecidable \cite{DBLP:journals/sLogica/MillerM05}. The main distinguishing feature regarding the decidability of $\POL$ resides in the fact that announcements in $\POL$ are not modal (agents observe atomic actions but not modal properties, e.g., `agent~$i$ knows~$p$'). Further connections 
% with $\BAPAL$ \cite{DBLP:journals/lmcs/DitmarschF22} can be explored as well.
% \FS{Compare with Heinemann 2007. François does not know what to say.}

